Implied Basket Correlation Dynamics

Equity basket correlation can be estimated both using the physical measure from stock prices, and also using the risk neutral measure from option prices. The difference between the two estimates motivates a so-called "dispersion strategy''. We study the performance of this strategy on the German market and propose several profitability improvement schemes based on implied correlation (IC) forecasts. Modelling IC conceals several challenges. Firstly the number of correlation coefficients would grow with the size of the basket. Secondly, IC is not constant over maturities and strikes. Finally, IC changes over time. We reduce the dimensionality of the problem by assuming equicorrelation. The IC surface (ICS) is then approximated from the implied volatilities of stocks and the implied volatility of the basket. To analyze the dynamics of the ICS we employ a dynamic semiparametric factor model.

==> README <==
                 The dgruyter package:                 
preparing books and journals for Walter de Gruyter GmbH


File:       README
Author:     le-tex publishing services


DESCRIPTION
===========

The dgruyter package assists in preparing manuscripts for de Gruyter
with {\LaTeX}. It provides some special commands for journal papers
as well as for books and generates the required appearance.
Together with corresponding font packages it allows to produce the 
final layout of De Gruyter books and journal articles.

COPYRIGHT
==========

Copyright:  (C) 2013 Walter de Gruyter GmbH

The ZIP file you have received, including the software, data, texts and 
fonts contained is provided to you under license from 
Walter de Gruyter GmbH, Genthiner Str. 13, 10785 Berlin, Germany

Your agreement to the copyright is assumed after you have become aware of them in your capacity as a user and have installed or
copied the dgruyter package or used them in any other way.
The dgruyter package is and shall remain the property of the Publisher and shall be used exclusively for the preparation of the Work by
you. You shall not use it for any other use, nor shall you sell or otherwise distribute the package.



FILES IN DISTRIBUTION
=====================

   BASE DISTRIBUTION:

      README                  This file.
      dgruyter.ins            Package installation file.
      dgruyter.dtx            Package source file.
      dg-degruyter.eps/.pdf   Logo files.
      dg-mouton.eps/.pdf      Logo files.
      dg-saur.eps/.pdf        Logo files.
      DG_attention.eps/.pdf   Vignette files.
      DG_exercise.eps/.pdf    Vignette files.
      DG_information.eps/.pdf Vignette files.
      DG_notice.eps/.pdf      Vignette files.
      DG_question.eps/.pdf    Vignette files.
      book.tex                Template file for a book.
      article.tex             Template file for a journal article.

   DOCUMENTATION:

      dgruyter.pdf            User manual for dgruyter package. 
                              It is produced as described below.


BASIC INSTALLATION
====================

   To get the package style file 'dgruyter.sty' and the
   index style files 'dgruyter.ist' and 'dgruyter.xdy' execute:
     latex dgruyter.ins

   The minimum requirement to use the package is to have
     dgruyter.sty and dgruyter.ist/dgruyter.xdy
     (as well as the logo and vignette files)
     in a directory where TeX can find it.

   To get the documentation 'dgruyter.pdf' execute:
     pdflatex dgruyter.dtx (at least twice)

